HUJI-KU at MRP~2020: Two Transition-based Neural Parsers

This paper describes the HUJI-KU system submission to the shared task on Cross-Framework Meaning Representation Parsing (MRP) at the 2020 Conference for Computational Language Learning (CoNLL), employing TUPA and the HIT-SCIR parser, which were, respectively, the baseline system and winning system in the 2019 MRP shared task. Both are transition-based parsers using BERT contextualized embeddings. We generalized TUPA to support the newly-added MRP frameworks and languages, and experimented with multitask learning with the HIT-SCIR parser. We reached 4th place in both the cross-framework and cross-lingual tracks.

==> Makefile <==
.PHONY: clean release

clean:
	rm *.aux *.log *.bbl *.blg *.out *~

release:
	-make clean;
	tar zpScvf ../../public/latex.tgz --transform='s@^@mrp/2019/latex/@'\
	  *


